$\sigma$-zero: Gradient-based Optimization of $\ell_0$-norm Adversarial Examples

Evaluating the adversarial robustness of deep networks to gradient-based attacks is challenging. While most attacks consider $\ell_2$- and $\ell_\infty$-norm constraints to craft input perturbations, only a few investigate sparse $\ell_1$- and $\ell_0$-norm attacks. In particular, $\ell_0$-norm attacks remain the least studied due to the inherent complexity of optimizing over a non-convex and non-differentiable constraint. However, evaluating adversarial robustness under these attacks could reveal weaknesses otherwise left untested with more conventional $\ell_2$- and $\ell_\infty$-norm attacks. In this work, we propose a novel $\ell_0$-norm attack, called $\sigma$-zero, which leverages a differentiable approximation of the $\ell_0$ norm to facilitate gradient-based optimization, and an adaptive projection operator to dynamically adjust the trade-off between loss minimization and perturbation sparsity. Extensive evaluations using MNIST, CIFAR10, and ImageNet datasets, involving robust and non-robust models, show that $\sigma$\texttt{-zero} finds minimum $\ell_0$-norm adversarial examples without requiring any time-consuming hyperparameter tuning, and that it outperforms all competing sparse attacks in terms of success rate, perturbation size, and efficiency.

==> tables/main_paper_fixed/fixed_k_cifar.tex <==
\begin{table}[htbp]
\caption{Fixed budget comparison results with 1000 steps on CIFAR10. See the caption of Table~\ref{tab:1k_maximum_budget_mnist} for further details.}
\label{tab:1k_maximum_budget_cifar}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.1}

\begin{tabular}{c|c|ccc|c|c|ccc|c}
\toprule
\textbf{Attack} & \textbf{M} & \textbf{ASR$_{24}$} & \textbf{ASR$_{50}$} & \textbf{ASR$_{100}$} & \textbf{q} & \textbf{M} & \textbf{ASR$_{24}$} & \textbf{ASR$_{50}$} & \textbf{ASR$_{100}$} & \textbf{q} \\ \hline


%C2C5
\PGDlzero & \multirow{5}{*}{\carmonshort} & 38.18 & 59.67 & 87.19 & 2.0 & \multirow{5}{*}{\croceloneshort} & 22.99 & 36.20 & 67.54 & 2.0 \\
Sparse-RS &  & 72.51 & 86.59 & 94.28 & 0.77 &  & 30.87 & 45.65 & 63.26 & 1.47 \\
\SPGDproj &  & 66.37 & 89.21 & 99.36 & 0.74 &  & 31.82 & 58.62 & 93.19 & 1.39 \\
\SPGDunproj &  & 66.33 & 91.07 & 99.75 & 0.72 &  & 36.16 & 70.06 & 98.07 & 1.30 \\
\cdashline{1-11} \sigmazero &  & \textbf{76.53} & \textbf{95.38} & \textbf{99.94} & 2.00 &  & \textbf{38.60} & \textbf{73.02} & \textbf{98.58} & 2.00 \\ \hline

%C3C10
\PGDlzero & \multirow{5}{*}{\augustinshort} & 32.41 & 59.19 & 89.22 & 2.0 & \multirow{5}{*}{\jiangloneshort} & 34.35 & 44.99 & 68.61 & 2.0 \\
Sparse-RS &  & 59.24 & 79.81 & 92.43 & 1.04 &  & 49.35 & 63.01 & 76.51 & 1.11 \\
\SPGDproj &  & 58.91 & 88.15 & 99.42 & 0.89 &  & 50.41 & 75.86 & 97.52 & 1.02 \\
\SPGDunproj &  & 64.8 & 93.15 & 99.92 & 0.76 &  & \textbf{55.89} & \textbf{84.64} & \textbf{99.56} & 0.91 \\
\cdashline{1-11} \sigmazero &  & \textbf{74.63} & \textbf{97.55} & \textbf{99.99} & 2.00 &  & 55.42 & 82.92 & 99.19 & 2.00 \\ \hline

%C4C9
\PGDlzero & \multirow{5}{*}{\engstromshort} & 37.91 & 68.90 & 95.31 & 2.0 & \multirow{5}{*}{\addepallishort} & 38.33 & 61.88 & 89.50 & 2.0 \\
Sparse-RS &  & 63.75 & 84.49 & 95.74 & 0.97 &  & 64.80 & 81.46 & 91.13 & 0.91 \\
\SPGDproj &  & 72.82 & 96.74 & 99.98 & 0.61 &  & 59.94 & 84.87 & 98.82 & 0.87 \\
\SPGDunproj &  & \textbf{81.64} & 99.09 & 100.0 & 0.42 &   & 65.07 & 90.78 & \textbf{99.83} & 0.75 \\
\cdashline{1-11} \sigmazero &  & 81.38 & \textbf{99.15} & 100.0 & 2.00 &  & \textbf{73.96} & \textbf{94.21} & 99.80 & 2.00 \\ \bottomrule

    
\end{tabular}
}
\end{table}

==> tables/main_paper_fixed/fixed_k_imagenet.tex <==
\begin{table*}[!h]
\centering
%\caption{Fixed budget comparison results with $N=1000$ ($N=2000$ for Sparse-RS to ensure fair comparison) on ImageNet. For each attack, we report the corresponding ASR with a feature budget level equal to 150. \revision{Remaining models in Appendix~\ref{appendix:additional_experiments}, Table~\ref{tab:1k_remaining_maximum_budget_imagenet}.}} 
\caption{Fixed budget comparison results with $N=1000$ ($N=2000$ for Sparse-RS) on ImageNet at a feature budget level $k = 150$. Remaining models in Appendix~\ref{appendix:additional_experiments}, \autoref{tab:1k_remaining_maximum_budget_imagenet}.}
\label{tab:1k_maximum_budget_imagenet}
\resizebox{\textwidth}{!}{%
%\setlength\tabcolsep{8.pt}
\renewcommand{\arraystretch}{1}
  \setlength\tabcolsep{20pt} 
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\multicolumn{1}{c}{\textbf{Attack}} & \multicolumn{1}{c}{\textbf{M}} & \multicolumn{1}{c}{\textbf{ASR$_{150}$}} & \multicolumn{1}{c}{\textbf{q}} & \multicolumn{1}{c}{\textbf{M}} & \multicolumn{1}{c}{\textbf{ASR$_{150}$}} & \multicolumn{1}{c}{\textbf{q}} \\ \hline
%I1I5
Sparse-RS & \multirow{4}{*}{\resnetvulnerableshort} & 91.5 & 0.34 & \multirow{4}{*}{\hendrycksshort} & 72.2 & 0.77 \\
\SPGDproj &  & 98.5 & 0.04 &   & 93.4 & 0.16 \\
\SPGDunproj &  & 97.8 & 0.05 & & 92.1 & 0.17 \\
\cdashline{1-7} \rc\sigmazero &  & \textbf{100.0} & 2.00 &  & \textbf{99.3} & 2.00 \\ \hline

%I2I6
Sparse-RS & \multirow{4}{*}{\engstromimagenetshort} & 84.1 & 0.49 & \multirow{4}{*}{\debenedettishort} & 47.4 & 1.15 \\
\SPGDproj &  & 91.2 & 0.2 &  & 74.9 & 0.55 \\
\SPGDunproj &  & 88.7 & 0.2 &   & 76.0 & 0.51 \\
\cdashline{1-7} \rc\sigmazero &  & \textbf{97.0} & 2.00 &  & \textbf{86.2} & 2.00 \\ \bottomrule



\end{tabular}

}
\end{table*}


==> tables/main_paper_fixed/fixed_k_mnist.tex <==
\begin{table}[htbp]
\caption{Fixed budget comparison results with $N=1000$ on MNIST. \revision{Sparse-RS was executed with double the steps, $2N$, to ensure fair comparison as it lacks backward passes.} For each attack, we report the corresponding ASR with different feature budget levels (24,50,100).}
\label{tab:1k_maximum_budget_mnist}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.1}

\begin{tabular}{c|c|ccc|c|c|ccc|c}
\toprule
\makecell{Attack} & \makecell{M} & \makecell{ASR$_{24}$} & \makecell{ASR$_{50}$} & \makecell{ASR$_{100}$} & \makecell{q} & \makecell{M} & \makecell{ASR$_{24}$} & \makecell{ASR$_{50}$} & \makecell{ASR$_{100}$} & \makecell{q} \\ \hline
\PGDlzero & \multirow{5}{*}{\smallcnnddnshort} & 73.99 & 99.90 & 100.0 & 2.0 & \multirow{5}{*}{\smallcnntradesshort} & 61.87 & 94.15 & 98.50 & 2.0 \\
Sparse-RS &  & 79.54 & 96.35 & 99.79 & 0.83 &  & \textbf{98.92} & 99.96 & 100.0 & 0.24 \\
\SPGDproj &  & 65.55 & 97.97 & 99.99 & 0.93 &  & 67.92 & 98.57 & 99.97 & 0.92 \\
\SPGDunproj &  & 82.79 & 99.65 & 100.0 & 0.46 &  & 62.25 & 98.11 & 99.99 & 1.0 \\
\cdashline{1-11} \sigmazero &  & \textbf{83.79} & \textbf{99.98} & 100.0 & 2.00 &  & 98.03 & \textbf{100.0} & 100.0 & 2.00 \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/main_paper_fixed/fixed_k_mnist_cifar.tex <==
\begin{table}[htb]
\caption{Fixed budget comparison results with $N=1000$ ($N=2000$ for Sparse-RS to ensure fair comparison) on MNIST and CIFAR10. For each attack, we report the corresponding ASR at feature budget levels $k=(24,50,100)$. Remaining models in Appendix~\ref{appendix:additional_experiments}, \autoref{tab:1k_remaining_maximum_budget_cifar}. }
\label{tab:1k_maximum_budget_mnist_cifar}
\resizebox{\textwidth}{!}{%
  \setlength\tabcolsep{8pt} 
\renewcommand{\arraystretch}{1.}

\begin{tabular}{c|c|ccc|c|c|ccc|c}

\toprule
\multicolumn{1}{c}{\textbf{Attack}} & \multicolumn{1}{c}{\textbf{M}} & \multicolumn{1}{c}{\textbf{ASR$_{24}$}} & \multicolumn{1}{c}{\textbf{ASR$_{50}$}} & \multicolumn{1}{c}{\textbf{ASR$_{100}$}} & \multicolumn{1}{c}{\textbf{q}} & \multicolumn{1}{c}{\textbf{M}} & \multicolumn{1}{c}{\textbf{ASR$_{24}$}} & \multicolumn{1}{c}{\textbf{ASR$_{50}$}} & \multicolumn{1}{c}{\textbf{ASR$_{100}$}} & \multicolumn{1}{c}{\textbf{q}} \\


\hline\hline
\multicolumn{11}{c}{MNIST} \\ \hline\hline


\PGDlzero & \multirow{5}{*}{\smallcnnddnshort} & 73.99 & 99.90 & 100.0 & 2.0 & \multirow{5}{*}{\smallcnntradesshort} & 61.87 & 94.15 & 98.50 & 2.0 \\
Sparse-RS &  & 79.54 & 96.35 & 99.79 & 0.83 &  & \textbf{98.92} & 99.96 & 100.0 & 0.24 \\
\SPGDproj &  & 65.55 & 97.97 & 99.99 & 0.93 &  & 67.92 & 98.57 & 99.97 & 0.92 \\
\SPGDunproj &  & 82.79 & 99.65 & 100.0 & 0.46 &  & 62.25 & 98.11 & 99.99 & 1.0 \\
\cdashline{1-11} \rc\sigmazero &  & \textbf{83.79} & \textbf{99.98} & 100.0 & 2.00 &  & 98.03 & \textbf{100.0} & 100.0 & 2.00 \\

\hline\hline
\multicolumn{11}{c}{CIFAR10} \\ \hline\hline

%C2C5
\PGDlzero & \multirow{5}{*}{\carmonshort} & 38.18 & 59.67 & 87.19 & 2.0 & \multirow{5}{*}{\croceloneshort} & 22.99 & 36.20 & 67.54 & 2.0 \\
Sparse-RS &  & 72.51 & 86.59 & 94.28 & 0.77 &  & 30.87 & 45.65 & 63.26 & 1.47 \\
\SPGDproj &  & 66.37 & 89.21 & 99.36 & 0.74 &  & 31.82 & 58.62 & 93.19 & 1.39 \\
\SPGDunproj &  & 66.33 & 91.07 & 99.75 & 0.72 &  & 36.16 & 70.06 & 98.07 & 1.30 \\
\cdashline{1-11} \rc\sigmazero &  & \textbf{76.53} & \textbf{95.38} & \textbf{99.94} & 2.00 &  & \textbf{38.60} & \textbf{73.02} & \textbf{98.58} & 2.00 \\ \hline

%C3C10
\PGDlzero & \multirow{5}{*}{\augustinshort} & 32.41 & 59.19 & 89.22 & 2.0 & \multirow{5}{*}{\jiangloneshort} & 34.35 & 44.99 & 68.61 & 2.0 \\
Sparse-RS &  & 59.24 & 79.81 & 92.43 & 1.04 &  & 49.35 & 63.01 & 76.51 & 1.11 \\
\SPGDproj &  & 58.91 & 88.15 & 99.42 & 0.89 &  & 50.41 & 75.86 & 97.52 & 1.02 \\
\SPGDunproj &  & 64.8 & 93.15 & 99.92 & 0.76 &  & \textbf{55.89} & \textbf{84.64} & \textbf{99.56} & 0.91 \\
\cdashline{1-11} \rc\sigmazero &  & \textbf{74.63} & \textbf{97.55} & \textbf{99.99} & 2.00 &  & 55.42 & 82.92 & 99.19 & 2.00 \\ \bottomrule

    


\end{tabular}
}
\end{table}

==> tables/main_paper_minimum/cifar_results.tex <==


%TABLE HACKS
\aboverulesep=0.2ex
\belowrulesep=0.2ex

\begin{table*}[!htb]
\caption{Minimum-norm comparison results for CIFAR10 with $N=1000$. See the caption of Table~\ref{tab:1k_minimum_norm_mnist} for further details. When VFGA exceeds the VRAM limit, we re-run it using a smaller batch size, increasing its runtime $t$. We denote those cases with the symbol `$\star$'.}
\label{tab:1k_minimum_norm_cifar}
\centering
\resizebox{1\textwidth}{!}{%
  \renewcommand{\arraystretch}{0.96}
\begin{tabular}{r|c|cccc|ccc|c|cccc|ccc}
\toprule
\textbf{Attack} & \textbf{M}& \textbf{ASR$_{10}$} & \textbf{ASR$_{50}$} & \textbf{ASR$_\infty$} & \medianlzero & $\mathbf{t}$ & $\mathbf{q}$  &\textbf{VRAM}& \textbf{M}& \textbf{ASR$_{10}$} & \textbf{ASR$_{50}$} & \textbf{ASR$_\infty$} & \medianlzero & $\mathbf{t}$ & $\mathbf{q}$  &\textbf{VRAM}\\ \midrule

% C2 C5
{SF} &  & 18.31 & 18.77 & 56.39 & 3072 & 11.31 & 1.40 & 1.62 && 15.89 & 24.36 & 58.29 & 3072 & 1.63 & 0.48 & 0.66 \\
{EAD} &  & 12.70 & 30.38 & 100.0 & 90 & 1.92 & 5.70 & 1.47 && 12.96 & 13.23 & 100.0 & 800 & 0.94 & 4.89 & 0.65  \\
{PDPGD} &  & 16.47 & 42.50 & 100.0 & 63 & 0.64 & 2.00 & 1.32 && 15.95 & 35.13 & 100.0 & 75 & 0.41 & 2.00 & 0.59 \\
{VFGA} &  & 28.98 & 75.37 & 99.92 & 24 & 0.59 & 0.78 & 11.71 &  & 18.86 & 49.98 & 99.72 & 51 & 0.32 & 1.25 & 4.44 \\
{BB} &  & 11.73 & 14.24 & 14.70 & \binfty & 0.63 & 2.05 & 1.47 && 14.13 & 22.91 & 27.64 & \binfty & 1.04 & 2.25 & 0.65 \\
{FMN} &  & 28.43 & 74.70 & 100.0 & 26 & 0.59 & 2.00 & 1.31 & & 18.61 & 48.87 & 100.0 & 52 & 0.24 & 2.00 & 0.60  \\
{BBadv} &  & 37.64 & 90.57 & 100.0 & 16 & 4.68 & 2.01 & 1.64 & & 19.93 & 72.43 & 100.0 & 34 & 5.28 & 2.01 & 0.64  \\
\cdashline{1-17}
{\sigmazero} & \multirow{-10}{*}{\textit \carmonshort} & \textbf{47.15} & \textbf{95.38} & 100.0 & \textbf{11} & 0.73 & 2.00 & 1.53 & \multirow{-10}{*}{\textit \croceloneshort} & \textbf{21.49} & \textbf{73.02} & \textbf{100.0} & \textbf{32} & 0.43 & 2.00 & 0.71 \\ \hline

{SF} &  & 14.30 & 21.22 & 98.74 & 3070 & 3.62 & 0.46 & 1.90 &  & 23.18 & 26.54 & 51.80 & 3072 & 0.58 & 0.33 & 0.51 \\
{EAD} &  & 9.21 & 11.42 & 100.0 & 360 & 2.53 & 5.62 & 1.89 &  & 15.75 & 29.23 & 100.0 & 118 & 1.01 & 5.32 & 0.41 \\
{PDPGD} &  & 13.96 & 45.15 & 100.0 & 55 & 1.12 & 2.00 & 1.8 &  & 19.43 & 41.00 & 100.0 & 66 & 0.44 & 2.00 & 0.36 \\
{VFGA} &  & 21.82 & 66.50 & 99.62 & 34 & 0.48 & 0.94 & 16.53 &  & 29.55 & 74.15 & 99.54 & 25 & 0.17 & 0.77 & 3.07 \\
{BB} &  & 21.32 & 56.78 & 58.64 & 33 & 2.31 & 2.89 & 1.89 &  & 38.64 & 91.83 & 100.0 & 15 & 10.90 & 2.93 & 0.41 \\
{FMN} &  & 20.61 & 71.70 & 100.0 & 33 & 1.08 & 2.00 & 1.8 &  & 29.75 & 73.71 & 100.0 & 26 & 0.41 & 2.00 & 0.36 \\
{BBadv} &  & 31.64 & 96.31 & 100.0 & 17 & 3.92 & 2.01 & 1.99 &  & 38.01 & 93.04 & 100.0 & 16 & 4.60 & 2.01 & 0.54 \\
\cdashline{1-17}
{\sigmazero} & \multirow{-10}{*}{\textit \augustinshort} & \textbf{36.61} & \textbf{97.55} & 100.0 & \textbf{15} & 1.41 & 2.00 & 1.92 & \multirow{-10}{*}{\textit \addepallishort} & \textbf{44.29} & \textbf{94.21} & 100.0 & \textbf{13} & 0.63 & 2.00 & 0.51 \\ \hline

% C4 C9
{SF} &  & 15.52 & 40.86 & 93.82 & 3039 & 9.3 & 1.56 & 1.90 &  & 26.85 & 43.07 & 91.14 & 69 & 4.32 & 1.49 & 0.66 \\
{EAD} &  & 9.48 & 11.14 & 100.0 & 398 & 2.57 & 5.66 & 1.89 &  & 23.94 & 24.78 & 100.0 & 768 & 1.04 & 4.99 & 0.65 \\
{PDPGD} &  & 15.50 & 49.19 & 100.0 & 51 & 1.16 & 2.00 & 1.8 &  & 26.89 & 42.38 & 100.0 & 66 & 0.40 & 2.00 & 0.60 \\
{VFGA} &  & 30.50 & 90.04 & 99.88 & 19 & 0.28 & 0.52 & 16.53 &  & 33.61 & 69.47 & 99.83 & 28 & 0.25 & 0.82 & 4.22 \\
{BB} &  & 16.32 & 31.03 & 31.36 & \binfty & 3.01 & 2.37 & 1.89 &  & 24.72 & 27.98 & 29.50 & \binfty & 0.54 & 2.09 & 0.65 \\
{FMN} &  & 26.85 & 85.60 & 100.0 & 23 & 1.09 & 2.00 & 1.8 &  & 32.63 & 62.96 & 100.0 & 34 & 0.35 & 2.00 & 0.59 \\
{BBadv} &  & 37.06 & 99.11 & 100.0 & 14 & 4.51 & 2.01 & 1.99 &  & 35.67 & 82.46 & 100.0 & 22 & 3.03 & 2.01 & 0.65 \\
\cdashline{1-17}
{\sigmazero} & \multirow{-10}{*}{\textit \engstromshort} & \textbf{42.96} & \textbf{99.15} & 100.0 & \textbf{12} & 1.39 & 2.00 & 1.91 & \multirow{-10}{*}{\textit \jiangloneshort} & \textbf{37.27} & \textbf{82.92} & 100.0 & \textbf{20} & 0.42 & 2.00 & 0.72 \\

\bottomrule

\end{tabular}
}
\end{table*}

==> tables/main_paper_minimum/imagenet_results.tex <==


%TABLE HACKS
\aboverulesep=0.2ex
\belowrulesep=0.2ex
\renewcommand{\arraystretch}{1.05}



\begin{table*}[htbp]
\caption{Minimum-norm comparison results for Imagenet with $N=1000$. See the caption of Table~\ref{tab:1k_minimum_norm_cifar} for further details.}
\label{tab:1k_minimum_norm_imagenet}
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{r|c|cccc|ccc|c|cccc|ccc}
\toprule
\textbf{Attack} & \textbf{M}& \textbf{ASR$_{10}$} & \textbf{ASR$_{50}$} & \textbf{ASR$_\infty$} & \medianlzero & $\mathbf{t}$ & $\mathbf{q}$  &\textbf{VRAM}& \textbf{M}& \textbf{ASR$_{10}$} & \textbf{ASR$_{50}$} & \textbf{ASR$_\infty$} & $ \medianlzero $ & $\mathbf{t}$ & $\mathbf{q}$  &\textbf{VRAM}\\ \midrule

%I1 I4
%EAD &  & 34.4 & 36.3 & 100.0 & 460 & 4.13 & 2.69 & 0.46 &  & 56.2 & 61.4 & 100.0 & 0 & 7.89 & 5.29 & 0.48 \\
%{VFGA} &  & 47.2 & 72.5 & 99.9 & 14 & 1.22$^\star$ & 1.08 & \color[HTML]{FF0000} > 40 &  & 61.6 & 76.6 & 99.3 & 0 & 1.74$^\star$ & 1.21 & \color[HTML]{FF0000} > 40 \\
%{FMN} &  & 48.7 & 81.0 & 100.0 & 12 & 0.73 & 2.00 & 0.66 &  & 63.8 & 78.7 & 100.0 & 0 & 0.72 & 2.00 & 0.67 \\
%{BBadv} &  & 55.9 & 93.2 & 100.0 & 7 & 231.67 & 2.01 & 0.72 &  & 70.4 & 89.6 & 100 & 0 & 199.47 & 2.01 & 0.73 \\
%\cdashline{1-17}
%{\sigmazero} & \multirow{-5}{*}{\textit \resnetvulnerableshort} & \textbf{62.0} & \textbf{95.9} & 100.0 & \textbf{5} & 1.18 & 2.00 & 0.84 & \multirow{-5}{*}{\textit \salmanshort} & \textbf{75.5} & \textbf{92.8} & 100.0 & 0 & 1.13 & 2.00 & 0.84 \\ \hline

%I2 I5
%{EAD} &  & 44.6 & 51.0 & 100.0 & 42 & 18.10 & 5.45 & 1.42 &  & 26.5 & 28.4 & 100.0 & 981 & 19.25 & 5.49 & 1.41 \\
%{VFGA} &  & 49.1 & 63.4 & 96.7 & 12 & 8.21$^\star$ & 2.35 & \color[HTML]{FF0000} > 40 &  & 36.6 & 59.5 & 97.9 & 31 & 6.93$^\star$ & 1.98 & \color[HTML]{FF0000} > 40 \\
%{FMN} &  & 50.9 & 67.0 & 100.0 & 9 & 1.97 & 2.00 & 2.30 &  & 38.1 & 67.7 & 100.0 & 25 & 1.98 & 2.00 & 2.30 \\
%{BBadv} &  & 57.5 & 82.3 & 100 & 4 & 182.65 & 2.01 & 2.40 &  & 44.3 & 85.5 & 100.0 & 14 & 205.11 & 2.01 & 2.41 \\
%\cdashline{1-17}
%{\sigmazero} & \multirow{-5}{*}{\textit \engstromimagenetshort} & \textbf{63.1} & \textbf{87.4} & 100.0 & \textbf{3} & 2.75 & 2.00 & 2.52 & \multirow{-5}{*}{\textit \hendrycksshort} & \textbf{46.6} & \textbf{86.9} & 100.0 & \textbf{13} & 2.76 & 2.00 & 2.52 \\ \hline

%I3 I6
%{EAD} &  & 55.1 & 60.2 & 100.0 & 0 & 21.38 & 5.50 & 1.41 &  & 32.3 & 33.5 & 100.0 & 572 & 11.43 & 5.34 & 1.68 \\
%{VFGA} &  & 62.2 & 76.2 & 98.8 & 0 & 6.11$^\star$ & 1.43 & \color[HTML]{FF0000} > 40 &  & 35.4 & 46.5 & 95.5 & 66 & 33.88$^\star$ & 3.97 & \color[HTML]{FF0000} > 40 \\
%{FMN} &  & 64.1 & 79.5 & 100.0 & 0 & 1.97 & 2.00 & 2.30 &  & 35.6 & 47.2 & 100.0 & 58 & 4.28 & 2.00 & 2.97 \\
%{BBadv} &  & 72.4 & 89.0 & 100.0 & 0 & 185.34 & 2.01 & 2.41 &  & 38.8 & 59..8 & 100.0 & 31 & 178.06 & 2.01 & 3.07 \\
%\cdashline{1-17}
%{\sigmazero} & \multirow{-5}{*}{\textit \wongshort} & \textbf{75.5} & \textbf{91.4} & 100.0 & 0 & 2.76 & 2.00 & 2.52 & \multirow{-5}{*}{\textit \debenedettishort} & \textbf{40.7} & \textbf{65.1} & 100.0 & \textbf{23} & 5.72 & 2.00 & 3.20 \\ \bottomrule

%I1 I5
EAD &  & 34.4 & 36.3 & 100.0 & 460 & 4.13 & 2.69 & 0.46 &  & 26.5 & 28.4 & 100.0 & 981 & 19.25 & 5.49 & 1.41 \\
{VFGA} &  & 47.2 & 72.5 & 99.9 & 14 & 1.22$^\star$ & 1.08 & \color[HTML]{FF0000} > 40  &  & 36.6 & 59.5 & 97.9 & 31 & 6.93$^\star$ & 1.98 & \color[HTML]{FF0000} > 40 \\
{FMN} &  & 48.7 & 81.0 & 100.0 & 12 & 0.73 & 2.00 & 0.66 &  & 38.1 & 67.7 & 100.0 & 25 & 1.98 & 2.00 & 2.30 \\
{BBadv} &  & 55.9 & 93.2 & 100.0 & 7 & 231.67 & 2.01 & 0.72 &  & 44.3 & 85.5 & 100.0 & 14 & 205.11 & 2.01 & 2.41 \\
\cdashline{1-17}
{\sigmazero} & \multirow{-5}{*}{\textit \resnetvulnerableshort} & \textbf{62.0} & \textbf{95.9} & 100.0 & \textbf{5} & 1.18 & 2.00 & 0.84 & \multirow{-5}{*}{\textit \hendrycksshort} & \textbf{46.6} & \textbf{86.9} & 100.0 & \textbf{13} & 2.76 & 2.00 & 2.52 \\ \hline

%I2 I6
{EAD} &  & 44.6 & 51.0 & 100.0 & 42 & 18.10 & 5.45 & 1.42 &  & 32.3 & 33.5 & 100.0 & 572 & 11.43 & 5.34 & 1.68 \\
{VFGA} &  & 49.1 & 63.4 & 96.7 & 12 & 8.21$^\star$ & 2.35 & \color[HTML]{FF0000} > 40 &  & 35.4 & 46.5 & 95.5 & 66 & 33.88$^\star$ & 3.97 & \color[HTML]{FF0000} > 40 \\
{FMN} &  & 50.9 & 67.0 & 100.0 & 9 & 1.97 & 2.00 & 2.30 &  & 35.6 & 47.2 & 100.0 & 58 & 4.28 & 2.00 & 2.97 \\
{BBadv} &  & 57.5 & 82.3 & 100 & 4 & 182.65 & 2.01 & 2.40 &  & 38.8 & 59..8 & 100.0 & 31 & 178.06 & 2.01 & 3.07 \\
\cdashline{1-17}
{\sigmazero} & \multirow{-5}{*}{\textit \engstromimagenetshort} & \textbf{63.1} & \textbf{87.4} & 100.0 & \textbf{3} & 2.75 & 2.00 & 2.52 & \multirow{-5}{*}{\textit \debenedettishort} & \textbf{40.7} & \textbf{65.1} & 100.0 & \textbf{23} & 5.72 & 2.00 & 3.20 \\ \bottomrule

\end{tabular}
    }
\end{table*}

==> tables/main_paper_minimum/mnist_results.tex <==

%TABLE HACKS
\aboverulesep=0.2ex
\belowrulesep=0.2ex
\renewcommand{\arraystretch}{1}

\begin{table*}[t]
\caption{Minimum-norm comparison results on MNIST with $N=1000$. For each attack and model ({M}), we report ASR at $k=10, 50, \infty$, median perturbation size \medianlzero, mean runtime $t$ (in seconds), mean number of queries $q$ ($\div$ 1000), and maximum VRAM usage (in GB).}
\label{tab:1k_minimum_norm_mnist}
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{r|c|cccc|ccc|c|cccc|ccc}
\toprule
\textbf{Attack} & \textbf{M}& \textbf{ASR$_{10}$} & \textbf{ASR$_{50}$} & \textbf{ASR$_\infty$} & \medianlzero & $\mathbf{t}$ & $\mathbf{q}$  &\textbf{VRAM}& \textbf{M}& \textbf{ASR$_{10}$} & \textbf{ASR$_{50}$} & \textbf{ASR$_\infty$} & \medianlzero & $\mathbf{t}$ & $\mathbf{q}$  &\textbf{VRAM}\\ \midrule
{SF} &  & 4.86 & 6.76 & 96.98 & 469 & 1.07 & 0.18 & 0.06 &  & 0.93 & 1.21 & 91.68 & 463 & 2.87 & 0.86 & 0.07 \\
EAD &  & 1.14 & 53.66 & 100.0 & 49 & 0.47 & 6.28 & 0.05 &  & 1.20 & 55.57 & 100.0 & 48 & 0.50 & 6.73 & 0.05 \\
{PDPGD} &  & 2.97 & 74.08 & 100.0 & 38 & 0.23 & 2.00 & 0.04 &  & 3.31 & 66.30 & 100.0 & 42 & 0.23 & 2.00 & 0.04 \\
{VFGA} &  & 9.62 & 82.42 & 99.98 & 27 & 0.05 & 0.77 & 0.21 &  & 1.80 & 39.33 & 99.95 & 57 & 0.05 & 1.33 & 0.21 \\
{BB} &  & 14.97 & 97.86 & 100.0 & 18 & 0.90 & 2.99 & 0.05 &  & 25.95 & 91.62 & 100.0 & 18 & 0.74 & 3.71 & 0.05 \\
{FMN} &  & 7.29 & 93.74 & 100.0 & 29 & 0.21 & 2.00 & 0.04 &  & 10.86 & 91.84 & 99.41 & 24 & 0.22 & 2.00 & 0.04 \\
{BBadv} &  & 14.81 & 91.23 & 100.0 & 19 & 0.77 & 2.01 & 0.07 &  & 14.42 & 40.88 & 100.0 & 89 & 0.71 & 2.01 & 0.07 \\
\cdashline{1-17}
{\sigmazero} & \multirow{-10}{*}{\textit{\smallcnnddnshort}} & \textbf{19.60} & \textbf{99.98} & 100.0 & \textbf{16} & 0.31 & 2.00 & 0.04 & \multirow{-10}{*}{\textit{\smallcnntradesshort}} & \textbf{61.57} & \textbf{100.0} & 100.0 & \textbf{9} & 0.31 & 2.00 & 0.04 \\ 
\bottomrule
\end{tabular}
}
\end{table*}
